From Inverse Optimization to Feasibility to ERM

Inverse optimization involves inferring unknown parameters of an optimization problem from known solutions and is widely used in fields such as transportation, power systems, and healthcare. We study the contextual inverse optimization setting that utilizes additional contextual information to better predict the unknown problem parameters. We focus on contextual inverse linear programming (CILP), addressing the challenges posed by the non-differentiable nature of LPs. For a linear prediction model, we reduce CILP to a convex feasibility problem allowing the use of standard algorithms such as alternating projections. The resulting algorithm for CILP is equipped with theoretical convergence guarantees without additional assumptions such as degeneracy or interpolation. Next, we reduce CILP to empirical risk minimization (ERM) on a smooth, convex loss that satisfies the Polyak-Lojasiewicz condition. This reduction enables the use of scalable first-order optimization methods to solve large non-convex problems while maintaining theoretical guarantees in the convex setting. Subsequently, we use the reduction to ERM to quantify the generalization performance of the proposed algorithm on previously unseen instances. Finally, we experimentally validate our approach on synthetic and real-world problems and demonstrate improved performance compared to existing methods.

==> App-QP-exp.tex <==
\section{\red{QP experiment}}
\label{app: QP-experiment}
This section presents our results for the Quadratic Program (QP) experiment. In this case, we consider the portfolio problem from the~\cref{sec:extension-nonlinear-constraints}. Recall the mathematical formulation of the problem described as: 


\begin{align}
\hat{x}(c) := \arg \min_{x \geq 0} -\langle c, x \rangle + \frac{\gamma}{2} x^{T} Q x \;\; \text{ s.t } \sum_{i=1}^{m} x_i = 1 
\label{eq:qp-def}
\end{align}

In this case, $x_j$ and $c_j$ represent the fraction of investment and the expected return for the stock $j \in [m]$, respectively.  The matrix $Q \in \mathbb{R}^{m\times m}$ represents the risk associated with selecting similar stocks,
and $\gamma$ is the given risk tolerance. The task is to maximize the return while minimizing the risk, subject to simplex constraints. 

\textbf{Dataset}: We generate the dataset following the codebase from~\cite{zharmagambetov2024landscape}. Following~\cite{zharmagambetov2024landscape}, we use $\gamma=0.1$ and $Q$ is assumed to be given to us as a part of the input. The dataset consists of $200$ training, validation and test samples. 


\textbf{Methods}: We compare our method revgrad(ERM) with QPTL~\cite{wilder2019melding}. We do not compare to other methods MOM, SPO+, BB and ST  from~\cref{sec:experiments} as they are designed exclusively for LPs.

\textbf{Setup}: We compare both methods in the deterministic setting with grid search for lr in $\{1.0, 0.1, 0.01, 0.001, 0.0001, 0.0001 \}$ for QPTL. We use armijo line search~\cite{armijo1966} for \texttt{revgrad}. We run both methods for two different model architectures: (1) single conv-2D and (2) two-layer conv-2D with ReLU non-linearity, and report our results for both.


\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{ICML 2024//Images/qp_estimate.png}
    \caption{Estimate Loss: \texttt{revgrad} outperforms QPTL for single layer and is slightly worse for $2$-layer case.}
        \label{fig:qp_estimate}
\end{figure}

\begin{figure}
        \centering
        \includegraphics[width=0.5\linewidth]{ICML 2024//Images/qp_decision.png}
        \caption{Decision Loss:\texttt{revgrad} outperforms QPTL for single layer and is slightly worse for $2$-layer case.}
        \label{fig:qp_decision}
    \end{figure}
    
\textbf{Results}: We plot the Estimate-Loss~\cref{eqn:estimate-loss} and Decision-Loss~\cref{eqn:decision-loss}  in~\cref{fig:qp_estimate} and ~\cref{fig:qp_decision} respectively. We can see that \texttt{revgrad} outperforms QPTL for a single layer and is worse for a $2$-layer case.



==> App-SSO.tex <==
\section{\red{SSO}}

Currently, the time taken to solve the QP~\cref{grad_inverse_lp_new} takes the majority of time during the training, taking $60$-$80\%$ of the total time. To amortize the cost of solving the QP, we can do multiple updates to the model parameters $\theta$ for a single solve of ~\cref{grad_inverse_lp_new}. For this, we incorporate the SSO\cite{lavington2023target} optimizer to form a surrogate which allows us to do multiple updates on the newly defined surrogate.

% Calculating the gradient of loss $h_2$, involves calculating the projection of targets by solving the QP. Solving this QP can be computationally expensive and become a bottleneck. This suboptimality has been studied in SSO \cite{lavington2023target}, where they proposed an optimizer in the case when calculating the gradient of loss is expensive. 

\textbf{Forming Surrogate}: In SSO, we define the surrogate on the target space, which is the predicted cost $c_i$ in our case. Let us define a loss $l$ in the target space. For $i^{th}$ index sample, $l_i$ for prediction target $c_i$ is defined as: $l_i(c_i) =  \arg \min_{q \in C_i} \|c_i-q\|^2$. Now we can use the loss $l$ to define the surrogate loss $g(\theta)$. At iteration $t$, $g_t(\theta)$ is defined as: $g_t(\theta)=  l_i(c_{i,t})+  \langle  \nabla l_i(c_{i,t}),\, f_{\theta}(z_{i,t})-c_{i,t} \rangle + \frac{1}{2\eta_t}\|f_{\theta}(z_{i,t}) - c_{i,t} \|^2$ where, $z_{i,t}$ denotes $i^{th}$ index is sampled at iteration $t$,  $c_{i,t}=f_{\theta_t}(z_{i,t})$ and $\eta_t$ is the learning rate at iteration $t$. 

\textbf{Advantage}: For surrogate $g_t(\theta)$, gradient computation of $g_t(\theta)$ is independent of the loss computation $l$ and thus gradient of $l$ which is bottleneck in our case. Thus, by doing multiple updates on $g_t{\theta}$, we can amortize the cost of computing $l$ and improve the computation efficiency of our framework.

\textbf{Experiments:} To compare the advantage of SSO, we compare a single update on $h(\theta)$ with multiple updates on $g_t{theta}$ with varying numbers of inner-iterations on $g$ and report the results in []. 

% Forming a surrogate at iteration $t$ , we get: 
% $g_t(\theta)= \frac{1}{n} \big[\sum_{i=1}^n l_i(p)+  \langle  \nabla l_i(p_t), f(\theta)-p_t \rangle + \frac{1}{2\eta}\|f(\theta) -p_t \|^2\big] $. As $\eta \leq \frac{1}{L}$, in our case, we can use $\eta=1$.



% Let us denote the target $Z\theta$ by $c$ for notation clarity. Also, let us also define a new loss $l$ in target space different from $h_2$. $l_i(c^i) = \arg \min_{q \in C_i} \|p^i-q\|^2$ where $p^i = Z_i \theta$ and $l(p) = \frac{1}{n} \sum_i l_i(p^i)$. 
% Also $p^*_t = \arg \min_{p \in \mathcal{P}}l_t(p)$ where $t$ denotes the iteration.


% In context of SSO, lets consider a loss $l_i(p) = h_2(p^i)$ where $p^i= f_i(\theta)$.  In the context of a linear model, $f_i(\theta) = Z_i \theta$. 


% Considering$y^i_t = \arg \min_{y} l_i(p_t)$ and $f_i(\theta) = Z^i \theta$. One step of the surrogate update gives us the following gradient:  

% \begin{align}
% \nabla g_t(\theta) &=  \frac{1}{n} \big[\sum_{i=1}^n 0 +  \langle  \nabla l_i(p_t), \nabla f(\theta) \rangle + \frac{1}{\eta}\|f(\theta) -p_t \|^2\big] \\
% \nabla g_t(\theta) &=  \frac{1}{n} \big[ \langle  \nabla l_i(p_t), \nabla f(\theta) \rangle + \frac{1}{\eta}\|0\|\big] \\
% \nabla g_t(\theta) &=  \frac{1}{n} (Z\theta-y)^T Z
% \end{align}

% % \unsure{How is our loss l strongly convex??}
% \begin{theorem}
%     (Theorem $4.2$ in \cite{lavington2023target}) Assuming that (i) $l_{i_t}$ is L-smooth and convex (ii) $l$ is $\mu$-strongly convex (iii) $p^*_t = \arg \min_{p_t \in \mathcal{P}} l_t(p)$ (iv) and, that for all $t$, $\epsilon_t \leq \epsilon$, $T$ iterations of SSO gives following bound for $p_T= f(\theta_T)$
    
%     $$\mathbb{E}\|p_{T+1} -p^*_{T+1}\| \leq \big( ( \Pi_{i=1}^T \rho_i) \|p_1-p^*_1\|^2  + 2\sigma^2\sum_{t=1}^T\Pi_{i=t+1}^T \rho_i \eta_t'^2  \big)^{\frac{1}{2}} + 2 \epsilon\sum_{t=1}^T\Pi_{i=t+1}^T \rho_i$$

%  where $\rho_t = (1-\mu\eta_t'), \sigma^2 =\mathbb{E}[\|\nabla l(p^*) - \nabla l_t(p^*) \|_2^2] $
 
%     % {Constant step size}:  When $\eta_t = \frac{1}{2Ln}$ and $\rho = 1- \frac{\mu}{2L}$
% \end{theorem}
% \begin{proof}
%     As $p^*$ is not a fixed point in our case, we can put our loss in the lemma $D.3$ in SSO paper and get the above bound. 
% \end{proof}

